Optimal Patient Allocation in Multi-Arm Clinical Trials

A multi-arm multi-stage trial is a multi-arm trial which includes interim analyses - analysing the data at certain specified points, generally discontinuing treatments which are concluded to not work and proceeding with the remainder. It is possible that the advantages of multi-arm trials over single-arm trials may be enhanced further by considering the allocation ratio, R. For an R:1 allocation ratio, Rn patients are allocated to the control arm and n patients allocated to each active treatment arm. In this study, the optimal allocation ratio will be defined as the allocation ratio which results in the smallest total sample size satisfying some required power and probability of type I error. This is an intuitive definition in the context of clinical trials, as a smaller trial will in general be more ethical and less expensive than a larger one satisfying the same error rates. The purpose of this paper is to investigate the optimal allocation ratio in the case of multiple active treatment arms. The setup for a single stage trial with K active treatment arms is described in Section 2, along with a brief exposition of Dunnett's statement regarding the optimal allocation ratio in such circumstances. Equations for type I error and power are derived, and the methodology used to investigate how total sample size may be minimised using allocation ratio is described. A two-stage trial is then considered, using the same methodology. Figures and tables showing how total sample size changes with allocation ratio, for a range of type I error and power values, are given in Section 3. The possible ethical and financial benefits of changing allocation ratio, including a simple example, is also included in Section 3. The results, and what they could mean in practical terms, are discussed in Section 4.

==> R.tex <==
\section{R code}

 \begin{landscape}


 \lstinputlisting{code.R}
 
 
\end{landscape}
 
 %\begin{lstlisting}
 % \end{lstlisting}

==> R2.tex <==


 \begin{landscape}
\section{R code}

 \lstinputlisting{newCODE.R}
 
 
\end{landscape}
 

==> abstract.tex <==

\clearpage
Hello - this is the abstract.

==> ackno.tex <==

\clearpage
Acknowledgements here.\\

Dominic Magirr, Lisa McNeill, Rachel Tribbick, John Whitehead and Thomas Jaki.

==> appx.tex <==
\clearpage

\chapter{Appendix}

%	\section{Appendix A: Dunnett's result}


%For a trial with multiple treatment arms, the probability of accepting the null hypothesis is
%\begin{eqnarray}
%1 - P(Z_M > c) & = & P(Z_1 < c , Z_2 < c, \dots , Z_k < c)\nonumber
%\label{eq:}
%\end{eqnarray}

%Maximising the probability of rejecting the null hypothesis, $P(Z_M > c)$, is of interest. (Back in 1955 XXX , this would have been pretty much impossible, so...) An approximation may be considered - a single test statistic $Z$, with power \\

%	\begin{equation}
%P(Z > c| H_A) \equiv P\left(\frac{\bar{X_1}-\bar{X_0}}{\sigma\sqrt{\frac{1}{n}+\frac{1}{RN}}} > c \right), \\
%\label{eq:x}
%\end{equation}

%where total sample size is $N = Rn + Kn$, with $Rn$ patients on the control treatment and $n$ patients on each of the $K$ treatments.\\

%Maximising the right hand side of (\ref{eq:xx}) is equivalent to minimising $\frac{1}{n} + \frac{1}{Rn}$. Now, $N = Rn + Kn \Leftrightarrow n = \frac{N}{R+K}$, therefore we can instead minimise $\frac{R+K}{N} + \frac{R+K}{RN}$:

%\begin{eqnarray}
%\frac{d}{dR} \left( \frac{R+K}{N} + \frac{R+K}{RN} \right) & = & 0 \nonumber \\
%\Rightarrow \frac{d}{dR} \left( \frac{R(R+K) + R + K}{RN}\right) & = & 0 \nonumber \\
%\Rightarrow \frac{d}{dR} \left( \frac{R}{N} +  \frac{K}{N} + \frac{1}{N} + \frac{K}{RN}\right) & = & 0 \nonumber \\
%\Rightarrow \frac{1}{N} - \frac{K}{R^2N} & = & 0 \nonumber \\
%\Rightarrow \frac{1}{N} & = & \frac{K}{R^2N}\nonumber \\
%\Rightarrow R^2 & = & \frac{KN}{N}\nonumber \\
%\Rightarrow R & = & \sqrt{K}\nonumber 			 
%\end{eqnarray}

%Hence, it may be argued from a theoretical perspective that the allocation ratio $\sqrt{K}:1$, if not exact, is at least a reasonable approximation.\\


	\section*{Appendix A: Type I equation}


%Consider a clinical trial with one control arm and $K$ active treatment arms, with an $R:1$ allocation ratio - that is, $Rn$ patients allocated to the control arm and $n$ patients allocated to each active treatment arm, giving a total sample size of $N = Rn + Kn$.

%The distribution of the mean of results for active treatment $i$ is\\

%\begin{equation}
%\bar{X_i} \sim (\mu_i, \frac{\sigma^2}{n}), i = 1, 2,\dotsc , k. \nonumber
%\label{eq:}
%\end{equation}

%The distribution of the sum of the results, $S_i = \sum_{j=1}^n X_{ij},  i = 1, 2,\dotsc , k, $  is then $S_i \sim (n\mu_i, n\sigma^2), i = 1, 2,\dotsc , k, $ for active treatments and $S_0 \sim (Rn\mu_i, Rn\sigma^2)$ for the control treatment.\\

%Consider the following test statistic for active treatment $i$: \\

%\begin{eqnarray}
%Z_i & \sim  &  N  \left(\frac{\bar{X_i} - \bar{X_0}}{\sigma \sqrt{\frac{R+1}{Rn}}}   \right) \nonumber\\
%		& =			&  \frac{\frac{S_i - S_0}{n}}{\sigma \sqrt{\frac{R+1}{Rn}}}\nonumber\\
%		& =			&	 \frac{S_i - S_0}{\sigma  \sqrt{\frac{R+1}{R}n}}
%\label{eq:sssss}
%\end{eqnarray}

%In trials with one active treatment arm, a Type I error is made when it is concluded to take the active treatment forward when its true treatment effect is below the minimum clinically relevant difference. For multi-armed trials, a type I error is made when at least one active treatment is taken forward erroneously. The decision to take the treatment forward is made if the test statistic for that treatment is greater than some critical value $c$. Therefore, a type I error is made if the greatest test statistic, denoted $Z_M$ exceeds the critical value $c$, given that the null hypothesis is true, and the probability of a Type I error occurring is

%			P \left(    \right) 

%\begin{eqnarray}
%\alpha  & = & P \left(  Z_M > c | H_0   \right) \nonumber \\
%\Rightarrow 1 - \alpha  & = & P \left(  Z_M < c | H_0   \right) \nonumber 
%\label{eq:}
%\end{eqnarray}

%$1-\alpha$ is then

\begin{eqnarray}
1-\alpha & = & P \left( Z_1 < c , Z_2 < c  \dotsc Z_K < c \right) \nonumber  \\
 & = & P \left(  \frac{RS_1 - S_0}{\sigma\sqrt{R(R+1)n}} < c , \frac{RS_2 - S_0}{\sigma\sqrt{R(R+1)n}} < c, \dotsc ,\frac{RS_K - S_0}{\sigma\sqrt{R(R+1)n}} < c  \right) \nonumber \\
 & = & P \left(  S_1 < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}, S_2 < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}, \dotsc, S_K < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}    \right) \nonumber
 \end{eqnarray}
 
These probabilities are not independent, as each depends on $S_K$. Therefore, condition on $S_0 (S_0 = s)$: 

\begin{eqnarray}
 & = & \int_{-\infty}^\infty \! P \left(  S_1 < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R},\dotsc , S_K < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R} \middle\vert S_0 = s  \right) f_{S_0}(s)  ds \nonumber  \\ 
 & = & \int_{-\infty}^\infty \! \prod_{i=1}^K P \left(  S_i < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R} \right) f_{S_0}(s)  ds \nonumber  \\ 
 & = & \int_{-\infty}^\infty \! \prod_{i=1}^K  P \left( \frac{S_i - n\mu_i}{\sqrt{n}\sigma} < \frac{1}{\sqrt{n}\sigma} \left(c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R} - n\mu_i \right)  \right)  f_{S_0}(s)  ds \nonumber  \\ 
 & = & \int_{-\infty}^\infty \! \prod_{i=1}^K  \Phi \left( c \sqrt{\frac{R+1}{R}} +  \frac{1}{\sqrt{n}\sigma} \left(\frac{s}{R}-n\mu_i \right)  \right) f_{S_0}(s)  ds. \nonumber  
%\label{eq:}
\end{eqnarray}


$f_{S_0}(s) = \frac{1}{\sqrt{Rn}\sigma} \phi \left(  \frac{s - Rn\mu_0}{\sqrt{Rn}\sigma}  \right)	$, thus $1-\alpha$ becomes


\begin{eqnarray}
 & = & \frac{1}{\sqrt{Rn}\sigma} \int_{-\infty}^\infty \! \prod_{i=1}^K \Phi \left( c \sqrt{\frac{R+1}{R}} +  \frac{1}{\sqrt{n}\sigma} \left(\frac{s}{R}-n\mu_i \right)  \right) \phi \left(  \frac{s - Rn\mu_0}{\sqrt{Rn}\sigma}  \right) ds \nonumber  
%\label{eq:}
\end{eqnarray}

Under $H_0$, $\mu_0 = \mu_1 = \dots = \mu_k = \mu $, therefore \\

\begin{eqnarray}
 & = & \frac{1}{\sqrt{Rn}\sigma} \int_{-\infty}^\infty \! \left[ \Phi \left( c \sqrt{\frac{R+1}{R}} +  \frac{1}{\sqrt{n}\sigma} \left( \frac{s}{R}-n\mu \right)  \right) \right]^K \phi \left(  \frac{s - Rn\mu}{\sqrt{Rn}\sigma}  \right) ds \nonumber  
%\label{eq:}
\end{eqnarray}

Set $x:= \frac{s - Rn\mu}{\sqrt{Rn}\sigma}$. Then $\frac{\partial x}{\partial s} = \frac{1}{\sqrt{Rn}\sigma}$, and \\

\begin{eqnarray}
%\setlength{\jot}{20pt} 
	\phi \left(  \frac{s - Rn\mu}{\sqrt{Rn}\sigma}  \right) ds & = & \phi (x) \frac{1}{|{\frac{\partial x}{\partial s}}|} \, dx 		\nonumber  \\ 
																														 & = & \sqrt{Rn}\sigma \phi (x)\, dx\text{, hence type I error can be expressed as} \nonumber  \\	
1 - \alpha & = & \int_{-\infty}^\infty \! \left[ 	\Phi \left(	c	\sqrt{\frac{R+1}{R}} + \frac{x}{\sqrt{R}} 	\right)		\right]^K \phi (x) dx \nonumber
%\label{eq:I}
\end{eqnarray}

as stated.

==> appx2.tex <==
\clearpage

\chapter{Appendix}

\section{Appendix A: Type I equation}

\begin{eqnarray}
1-\alpha & = & P \left( Z_1 < c , Z_2 < c  \dotsc Z_K < c \right) \nonumber  \\
 & = & P \left(  \frac{RS_1 - S_0}{\sigma\sqrt{R(R+1)n}} < c , \frac{RS_2 - S_0}{\sigma\sqrt{R(R+1)n}} < c, \dotsc ,\frac{RS_K - S_0}{\sigma\sqrt{R(R+1)n}} < c  \right) \nonumber \\
 & = & P \left(  S_1 < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}, S_2 < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}, \dotsc, S_K < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}    \right) \nonumber
 \end{eqnarray}
 
These probabilities are not independent, as each depends on $S_K$. Therefore, condition on $S_0 (S_0 = s)$: 

\begin{eqnarray}
 & = & \int_{-\infty}^\infty \! P \left(  S_1 < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R},\dotsc , S_K < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R} \middle\vert S_0 = s  \right) f_{S_0}(s)  ds \nonumber  \\ 
 & = & \int_{-\infty}^\infty \! \prod_{i=1}^K P \left(  S_i < c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R} \right) f_{S_0}(s)  ds \nonumber  \\ 
 & = & \int_{-\infty}^\infty \! \prod_{i=1}^K  P \left( \frac{S_i - n\mu_i}{\sqrt{n}\sigma} < \frac{1}{\sqrt{n}\sigma} \left(c\sigma \sqrt{\frac{R+1}{R}n} + \frac{s}{R} - n\mu_i \right)  \right)  f_{S_0}(s)  ds \nonumber  \\ 
 & = & \int_{-\infty}^\infty \! \prod_{i=1}^K  \Phi \left( c \sqrt{\frac{R+1}{R}} +  \frac{1}{\sqrt{n}\sigma} \left(\frac{s}{R}-n\mu_i \right)  \right) f_{S_0}(s)  ds. \nonumber  
%\label{eq:}
\end{eqnarray}


$f_{S_0}(s) = \frac{1}{\sqrt{Rn}\sigma} \phi \left(  \frac{s - Rn\mu_0}{\sqrt{Rn}\sigma}  \right)	$, thus $1-\alpha$ becomes


\begin{eqnarray}
 & = & \frac{1}{\sqrt{Rn}\sigma} \int_{-\infty}^\infty \! \prod_{i=1}^K \Phi \left( c \sqrt{\frac{R+1}{R}} +  \frac{1}{\sqrt{n}\sigma} \left(\frac{s}{R}-n\mu_i \right)  \right) \phi \left(  \frac{s - Rn\mu_0}{\sqrt{Rn}\sigma}  \right) ds \nonumber  
%\label{eq:}
\end{eqnarray}

Under $H_0$, $\mu_0 = \mu_1 = \dots = \mu_k = \mu $, therefore \\

\begin{eqnarray}
 & = & \frac{1}{\sqrt{Rn}\sigma} \int_{-\infty}^\infty \! \left[ \Phi \left( c \sqrt{\frac{R+1}{R}} +  \frac{1}{\sqrt{n}\sigma} \left( \frac{s}{R}-n\mu \right)  \right) \right]^K \phi \left(  \frac{s - Rn\mu}{\sqrt{Rn}\sigma}  \right) ds \nonumber  
%\label{eq:}
\end{eqnarray}

Set $x:= \frac{s - Rn\mu}{\sqrt{Rn}\sigma}$. Then $\frac{\partial x}{\partial s} = \frac{1}{\sqrt{Rn}\sigma}$, and \\

\begin{eqnarray}
%\setlength{\jot}{20pt} 
	\phi \left(  \frac{s - Rn\mu}{\sqrt{Rn}\sigma}  \right) ds & = & \phi (x) \frac{1}{|{\frac{\partial x}{\partial s}}|} \, dx 		\nonumber  \\ 
																														 & = & \sqrt{Rn}\sigma \phi (x)\, dx\text{, hence type I error can be expressed as} \nonumber  \\	
1 - \alpha & = & \int_{-\infty}^\infty \! \left[ 	\Phi \left(	c	\sqrt{\frac{R+1}{R}} + \frac{x}{\sqrt{R}} 	\right)		\right]^K \phi (x) dx \nonumber
%\label{eq:I}
\end{eqnarray}

as stated.

\section{Appendix B: Power equation}


\begin{eqnarray}
1 - \beta & = & P(\text{Proceed with treatment } K | H_A:= \mu_0 =0, \mu_1 = \mu_2 = \dots = \mu_{K-1} = \delta_0, \mu_K = \delta)\nonumber\\
		& = & P(Z_K > C, Z_K = Z_M |H_A)\nonumber\\
 & = & P \left(	Z_K > C, Z_1 < Z_K, Z_2 < Z_K, \dotsc , Z_{K-1} < Z_K	 | H_A	\right) \nonumber \\
 				& = & P \left(		\frac{RS_K - S_0}{\sigma  \sqrt{R(R+1)n}}	> C , \, \frac{RS_1 - S_0}{\sigma  \sqrt{R(R+1)n}}	< \frac{RS_K - S_0}{\sigma  \sqrt{R(R+1)n}}, \right. \nonumber \\
 				&   &  \left. \frac{RS_2 - S_0}{\sigma  \sqrt{R(R+1)n}}	< \frac{RS_K - S_0}{\sigma  \sqrt{R(R+1)n}}	, \dotsc , \frac{RS_{K-1} - S_0}{\sigma  \sqrt{R(R+1)n}}	< \frac{RS_K - S_0}{\sigma  \sqrt{R(R+1)n}} \middle\vert H_A \right) \nonumber \\
 				& = & P \left(	S_K > C\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	, S_1 < S_K , S_2 < S_K , \dotsc , S_{K-1} < S_K  \middle\vert H_A	\right) \nonumber
%\label{eq:}
\end{eqnarray}

Again, these probabilities are not independent. Condition on $S_0 (= s_0)$ and $S_K (= s_K)$: 

\begin{eqnarray}
 & = & \int_{-\infty}^{\infty}	\int_{C\sigma \sqrt{\frac{R+1}{R}n} + \frac{s_0}{R}	}^\infty \! \prod_{i=1}^{K-1} P ( S_i < s_k | S_0 = s_0, S_K = s_K, H_A) f_{S_0}(s_0) f_{S_K}(s_K)	ds_K ds_0 \nonumber
%\label{eq:}
\end{eqnarray}

$ f_{S_0}(s_0)	= \frac{1}{\sigma \sqrt{Rn}} \phi \left(  \frac{s_0 - Rn\mu_0}{\sigma \sqrt{Rn}}		\right)$ and $ f_{S_K}(s_K)	= \frac{1}{\sigma \sqrt{n}} \phi \left(  \frac{s_K - n\mu_K}{\sigma \sqrt{n}}		\right)$, so $1 - \beta$ is then 

\begin{eqnarray}
 & = & \frac{1}{\sigma^2 n \sqrt{R}} \int_{-\infty}^{\infty}	\int_{C\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	}^\infty \! \prod_{i=1}^{K-1} P ( S_i < s_k |  S_0 = s_0, S_K = s_K, H_A) \nonumber\\
 & & \times \phi \left(  \frac{s_0 - Rn\mu_0}{\sigma \sqrt{Rn}}	\right) \phi \left(  \frac{s_K - n\mu_K}{\sigma \sqrt{n}}	\right)		ds_K ds_0 \nonumber\\
 & = & \frac{1}{\sigma^2 n \sqrt{R}} \int_{-\infty}^{\infty}	\int_{C\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	}^\infty \! \prod_{i=1}^{K-1} P \left(\frac{S_i - n\mu_i}{\sigma \sqrt{n}} <	\frac{s_K - n\mu_i}{\sigma \sqrt{n}}  \middle\vert S_0 = s_0, S_K = s_K, H_A\right) \nonumber\\
 & & \times \phi \left(  \frac{s_0 - Rn\mu_0}{\sigma \sqrt{Rn}}	\right) \phi \left(  \frac{s_K - n\mu_K}{\sigma \sqrt{n}}	\right)		ds_K ds_0 \nonumber
\end{eqnarray}

Under $H_A, \mu_0 = 0, \mu_1 = \mu_2 = \dots = \mu_{K-1} = \delta_0, \mu_K = \delta$, giving\\

\begin{eqnarray}
& = & \frac{1}{\sigma^2 n \sqrt{R}} \int_{-\infty}^{\infty}	\int_{C\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	}^\infty \! \left[ \Phi \left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} \right) \right]^{K-1}  \phi \left(  \frac{s_0}{\sigma \sqrt{Rn}}	\right) \phi \left(  \frac{s_K - n\delta}{\sigma \sqrt{n}}	\right)		ds_K ds_0 \nonumber
\end{eqnarray}

Changing order of integration:
\begin{eqnarray}
& = & \frac{1}{\sigma^2 n \sqrt{R}} \int_{-\infty}^{\infty}	\int_{-\infty}^{RS_K - C \sigma \sqrt{R(R+1)}n}  \! \left[ \Phi \left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} \right) \right]^{K-1}  \phi \left(  \frac{s_0}{\sigma \sqrt{Rn}}	\right) \phi \left(  \frac{s_K - n\delta}{\sigma \sqrt{n}}	\right)		ds_0 ds_K \nonumber\\
& = & \frac{1}{\sigma \sqrt{n}} \int_{-\infty}^{\infty} \! \Phi \left( \frac{RS_K - C \sigma \sqrt{R(R+1)}n}{\sigma \sqrt{Rn}}	\right) 	\left[ \Phi \left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} \right) \right]^{K-1}  \phi \left(  \frac{s_K - n\delta}{\sigma \sqrt{n}}	\right)	ds_K \nonumber
\end{eqnarray}


%   & = &  \frac{1}{\sigma \sqrt{n}} 	\int_{c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	}^\infty \!   \left[ \Phi	\left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} 	\right)	\right]^{K-1}	\phi \left(\frac{S_K - n\delta}{\sigma \sqrt{n}} 	\right)	ds_K \nonumber \\
%   & = &  \frac{1}{\sigma \sqrt{n}} \int_{-\infty}^{\infty}	\int_{c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	}^\infty \left[ \Phi	\left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} 	\right)	\right]^{K-1}	\phi \left(\frac{S_K - n\delta}{\sigma \sqrt{n}} 	\right)	f_{S_0}(s_0) ds_K ds_0 \nonumber \\
 %  & = & \frac{1}{\sigma^2 n \sqrt{R}}	\int_{-\infty}^{\infty}	\int_{c\sigma \sqrt{\frac{R+1}{R}n} + \frac{S_0}{R}	}^\infty \left[ \Phi	\left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} 	\right)	\right]^{K-1}	\phi \left(\frac{S_K - n\delta}{\sigma \sqrt{n}} 	\right)	\phi \left( \frac{S_0}{\sigma \sqrt{Rn}}  \right) ds_K ds_0 \nonumber \\
  % & = & \frac{1}{\sigma^2 n \sqrt{R}}	\int_{-\infty}^{\infty}	\int_{-\infty}^{RS_K - c \sigma \sqrt{R(R+1)}n} \left[ \Phi	\left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} 	\right)	\right]^{K-1}	\phi \left(\frac{S_K - n\delta}{\sigma \sqrt{n}} 	\right)	\phi \left( \frac{S_0}{\sigma \sqrt{Rn}}  \right) ds_0 ds_K \nonumber \\
  % & = & \frac{1}{\sigma \sqrt{n}} \int_{-\infty}^{\infty} \left[ \Phi	\left(\frac{s_K - n\delta_0}{\sigma \sqrt{n}} 	\right)	\right]^{K-1} \Phi \left(		\frac{RS_K - c\sigma \sqrt{R(R+1)n}}{\sigma \sqrt{Rn}}		\right) \phi \left(\frac{S_K - n\delta}{\sigma \sqrt{n}} 	\right) ds_K. \nonumber
%\label{eq:}
%\end{eqnarray}

Setting $w: = \frac{s_K - n\delta}{\sigma \sqrt{n}}, \Rightarrow \frac{\partial w}{\partial s_K} = \frac{1}{\sigma \sqrt{n}} $\\

$\Rightarrow \phi \left(  \frac{s_K - n\delta}{\sigma \sqrt{n}}	\right) ds_K = \frac{1}{\left|	\frac{\partial w}{\partial s_K}		\right|} \phi(w) dw = \sigma \sqrt{n} \phi(w) \,dw$, thus\

\begin{eqnarray}
1 - \beta		& = & \int_{-\infty}^{\infty} \Phi \left( w \sqrt{R} + \frac{\sqrt{Rn}\delta}{\sigma} - C \sqrt{R+1} \right) \left[  \Phi  \left(	 w + \frac{\sqrt{n}}{\sigma} (\delta - \delta_0)	\right) \right]^{K-1} \phi(w) \,dw \nonumber
%\label{eq:t2}
\end{eqnarray}

 
 
 
 \clearpage


\section{Appendix C: Further results}
				
 				

\begin{figure}[!h]
  \begin{center}
   \subfigure[Active treatments = 2]{\label{fig:sigk2}\includegraphics[scale=0.41]{sigk2.pdf}}
    \subfigure[Active treatments = 3]{\label{fig:sigk3}\includegraphics[scale=0.41]{sigk3.pdf}}
     \subfigure[Active treatments = 4]{\label{fig:sigk4}\includegraphics[scale=0.41]{sigk4.pdf}}
      \subfigure[Active treatments = 5]{\label{fig:sigk5}\includegraphics[scale=0.41]{sigk5.pdf}}
  \end{center}
  \caption{Change in total sample size for $ \sigma = 1, 1.25, 1.5, 1.75$ and $K = 2, 3, 4, 5$, with fixed arguments $\alpha = 0.05,$ power $= 0.9, \delta = 0.5,$ and $\delta_0 = 0.125$}
  \label{fig:sig}
  \end{figure}
  
\begin{figure}[!h]
  \begin{center}
   \subfigure[Active treatments = 2]{\label{fig:dk2}\includegraphics[scale=0.41]{dk2.pdf}}
    \subfigure[Active treatments = 3]{\label{fig:dk3}\includegraphics[scale=0.41]{dk3.pdf}}
     \subfigure[Active treatments = 4]{\label{fig:dk4}\includegraphics[scale=0.41]{dk4.pdf}}
      \subfigure[Active treatments = 5]{\label{fig:dk5}\includegraphics[scale=0.41]{dk5.pdf}}
  \end{center}
  \caption{Change in total sample size for $ \delta = 0.5, 0.6, 0.7, 0.8$ and $K = 2, 3, 4, 5$, with fixed arguments $\alpha = 0.05,$ power $= 0.9, \sigma = 1$ and $\delta_0 = 0.125$}
  \label{fig:d}
  \end{figure}
  
   
\begin{figure}[!h]
  \begin{center}
   \subfigure[Active treatments = 2]{\label{fig:d0k2}\includegraphics[scale=0.41]{d0k2.pdf}}
    \subfigure[Active treatments = 3]{\label{fig:d0k3}\includegraphics[scale=0.41]{d0k3.pdf}}
     \subfigure[Active treatments = 4]{\label{fig:d0k4}\includegraphics[scale=0.41]{d0k4.pdf}}
      \subfigure[Active treatments = 5]{\label{fig:d0k5}\includegraphics[scale=0.41]{d0k5.pdf}}
  \end{center}
  \caption{Change in total sample size for $ \delta_0 = 0.075, 0.125, 0.175, 0.225$ and $K = 2, 3, 4, 5$, with fixed arguments $\alpha = 0.05,$ power $= 0.9, \sigma = 1$ and $\delta = 0.5$}
  \label{fig:d0}
  \end{figure}
  
  

==> bigtable.tex <==

  \begin{landscape}
  \begin{table}[htb]
	\centering
		\begin{tabular}{ccc|cc cc cc cc}
		& & & \multicolumn{8}{c}{Active treatments $K$}\\
		 & &  & \multicolumn{2}{c}{2 } & \multicolumn{2}{c}{3 }& \multicolumn{2}{c}{4 }& \multicolumn{2}{c}{5 } \\
	     \hline
	    & & $1 - \beta$					 					& 0.8 			& 0.9		& 0.8	 	& 0.9		& 0.8	 	& 0.9		& 0.8 		& 0.9\\
	     \hline
	     & & $R$ 											&				&			&			&			&			&			&			&\\		
	     \multirow{12}{*}{$\alpha$}& \multirow{3}{*}{0.2} & 1$(N)$	& 108			& 159 		& 172		& 244		& 240		& 335		& 312		& 432\\
	     &&2												&1.07 (-8)		& 1.08 (-13)	& 1.05 (-8)	& 1.05 (-11)	& 1.00 (0)	&1.00 (-1)	& 0.99 (4)	&0.99 (5)\\
	     &&$R_{op}$										&1.00 (0) 		& 0.99 (2)	& 1.00 (0)	& 0.99 (3)	& 0.98 (4)	&0.98 (6)		& 0.97 (10)	&0.96 (16)\\
	     &&&&&&&&&&\\
	      					& \multirow{3}{*}{0.1} & 1$(N)$	& 147			& 204		& 224		& 304		& 305		& 410		& 390			& 516\\
	     &&2												& 1.03 (5)		& 1.04 (-8)	& 1.00 (-1)	&1.00 (-1)	& 0.96 (11)	&0.97 (14)	&0.94 (24)		& 0.95 (26)\\
	     &&$R_{op}$										& 0.99 (1)		& 0.99 (2)	& 0.98 (5)	&0.98 (7)		& 0.95 (15)	&0.95 (19)	&0.95 (19)		& 0.95 (28)\\
 &&&&&&&&&&\\
	      					& \multirow{3}{*}{0.05} & 1$(N)$	& 186			& 249		& 276		& 364		& 370		& 485		& 468		& 606\\
	     &&2												&1.03 (-6)		& 1.03 (-7)	&0.98 (6)		& 0.98 (9)	&0.94 (22)	& 0.94 (29)	& 0.93 (34)	&0.92 (46)\\
	     &&$R_{op}$    										&0.99 (2)			& 0.99 (2)	&0.96 (10)	& 0.96 (14)	& 0.94 (22)	&0.94 (30)	& 0.92 (37)	&0.92 (48)\\
 &&&&&&&&&&\\
	      					& \multirow{3}{*}{0.025} & 1$(N)$	& 228			& 297		& 332 		& 428		 & 440		& 560		& 552	& 702\\
	     &&2												& 1.02 (-4)		&1.01 (-3)	&0.96 (12)	&0.96 (18)	&0.93 (32)	&0.93 (38		&0.90 (55)& 0.91 (65)\\
	     &&$R_{op}$										&0.97 (6)			&0.97 (8)		&0.95 (17)	&0.95(23)		&0.92 (35)	&0.93 (41)	&0.90 (55)&0.90 (70)\\

		\end{tabular}
	\caption{Reduction in sample size achieved by choosing $R=2$ or $R=R_{op}$, compared to $R=1$. Reduction given by proportion and number (where proportion $>1$ indicates \textit{increase} in sample size)}
	\label{tab:gains}
\end{table}
\end{landscape}


\begin{table}[htbp]
	\centering
		\begin{tabular}{cc|cccc}
		&	&	\multicolumn{4}{c}{$\alpha$}\\
		&	&			     0.2		& 0.1	& 0.05	  & 0.025 \\
		\hline
		\multirow{4}{*}{$K$}& 2 & 0.99 (2) & 0.99 (2) & 0.99 (2)  &0.97 (8) \\
						& 3 & 0.99 (3) & 0.97 (9) & 0.96 (14) &0.95(23)\\
						& 4 & 0.98 (6) & 0.95 (19)& 0.94 (30) &0.93 (41)\\
						& 5 & 0.96 (16)& 0.95 (28)& 0.92 (48) &0.90 (70)\\			
		\end{tabular}
	\caption{OLD TABLE: Sample size reduction achieved by choosing optimal allocation ratio, as a proportion of sample size for $1:1$ ratio (actual reduction in brackets)}
	\label{tab:1}
\end{table}

 \begin{table}[htbp]
	\centering
		\begin{tabular}{cc|cc}
		&	&	\multicolumn{2}{c}{Power}\\
		&	&	0.8	& 0.9 \\
		\hline
		\multirow{4}{*}{$K$}& 2 & 0.99 (2) & 0.99 (2)  \\
						& 3 & 0.96 (10) & 0.96 (14)  \\
						& 4 & 0.94 (22) & 0.94 (30) \\
						& 5 & 0.92 (37)& 0.92 (48) \\			
		\end{tabular}
	\caption{OLD POWER TABLE :Sample size reduction achieved by choosing optimal allocation ratio, as a proportion of sample size for $1:1$ ratio (actual reduction in brackets)}
	\label{tab:2}
\end{table}


\begin{table}[htb]
	\centering
		\begin{tabular}{cc|cc cc cc cc}
		& & \multicolumn{8}{c}{ \textbf{Active treatments} $\mathbf{K}$}\\
	     & & \multicolumn{2}{c}{2 } & \multicolumn{2}{c}{3 }& \multicolumn{2}{c}{4}& \multicolumn{2}{c}{5} \\
	     \hline
	     & $\mathbf{1 - \beta}$ 			 		& 0.8 	& 0.9	& 0.8 	& 0.9	& 0.8 	& 0.9	& 0.8 	& 0.9\\
	     \hline
	     &&&&&&&&&\\
	     \multirow{4}{*}{$\mathbf{\alpha}$} & \textbf{0.2}	& 1.5	& 1.7	& 1.9	& 1.9	& 2.3	& 2.2	& 2.8	& 2.7\\
	      &&&&&&&&&\\
	      & \textbf{0.1}						& 2.0	& 1.9	& 2.5	& 2.4	& 3.0	& 2.9	& 3.7	& 3.4\\
	      &&&&&&&&&\\
	      & \textbf{0.05}						& 2.0	& 2.0	& 2.7	& 2.6	& 3.3	& 3.3	& 4.3	& 4.0\\
	      &&&&&&&&&\\
	      & \textbf{0.025}						& 2.1	& 2.2	& 3.0	& 2.9	& 3.8	& 3.7	& 4.6	& 4.5\\
		\end{tabular}
	\caption{Maximum allocation ratios do not result in a sample size increase of $ > 3\% $ compared to $R=1$ } %$(\sigma = 1, \delta = 0.5, \delta_0 = 0.125)$ }
	\label{tab:maxR}
\end{table}
% BIG MAX ALLOCATION RATIO TABLE

==> declaration.tex <==
\clearpage

Ernest Borgnine wrote this entire thesis without any help from his supervisor, who was a useless sod.

 %space for signature 
 \vspace{2in}

Ernest Borgnine

 %space for supervisor's signature 
 \vspace{2in}

Stephen Hawking
